The Fast Loaded Dice Roller: A Near-Optimal Exact Sampler for Discrete Probability Distributions

This paper introduces a new algorithm for the fundamental problem of generating a random integer from a discrete probability distribution using a source of independent and unbiased random coin flips. We prove that this algorithm, which we call the Fast Loaded Dice Roller (FLDR), is highly efficient in both space and time: (i) the size of the sampler is guaranteed to be linear in the number of bits needed to encode the input distribution; and (ii) the expected number of bits of entropy it consumes per sample is at most 6 bits more than the information-theoretically optimal rate. We present fast implementations of the linear-time preprocessing and near-optimal sampling algorithms using unsigned integer arithmetic. Empirical evaluations on a broad set of probability distributions establish that FLDR is 2x-10x faster in both preprocessing and sampling than multiple baseline algorithms, including the widely-used alias and interval samplers. It also uses up to 10000x less space than the information-theoretically optimal sampler, at the expense of less than 1.5x runtime overhead.

==> figures/alg-alias.tex <==
%!TEX root=../paper.tex
\begin{algorithm}[t]
\caption{\footnotesize Alias sampling}
\label{alg:alias}
\begin{algorithmic}[1]
\footnotesize
% \Require Positive integers $(a_1, \dots, a_n)$, $m \defas \sum_{i=1}^{n}a_i$.
% \Ensure Random integer $i$ with probability $a_i / m$.
%
\Statex \texttt{// PREPROCESS}
  \label{algline:-uniform-preprocess}
\State Build alias table $(q, j)$ (\citet[III.4]{devroye1986})
%
\Statex \texttt{// SAMPLE}
\State $i \sim \textsc{FastDiceRoller}(n)$; (\citet[p.~4]{lumbroso2013})
    \label{algline:alias-fdr}
\State $x \sim \textsc{Bernoulli}(q[i])$; (\citet[p.~21]{lumbroso2013})
  \label{algline:alias-bernoulli}
\If{$(x = 1)$} \{\Return $i$;\} \algorithmicelse\ \{\Return $j[i]$;\} \EndIf
\end{algorithmic}
\end{algorithm}


==> figures/dimension-rate.tex <==
%!TEX root=../paper.tex
\begin{figure*}[ht]
\begin{subfigure}{.5\linewidth}
\includegraphics[width=\linewidth]{assets/dimension-rate-cpp.pdf}
\captionsetup{size=footnotesize, skip=0pt}
% \caption{Sampling Runtime}
% \label{fig:dimension-rate}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
\includegraphics[width=\linewidth]{assets/dimension-preprocess-cpp.pdf}
\captionsetup{size=footnotesize, skip=0pt}
% \caption{Preprocessing Runtime}
% \label{fig:dimension-preprocess}
\end{subfigure}
\caption{
Comparison of sampling runtime (left) and  preprocessing runtime
  (right) with varying dimensionality $n$ of the target distribution,
  according to FLDR (red) and baseline approximate sampling
  algorithms.}
\medskip
\end{figure*}


==> figures/entropy-rate.tex <==
%!TEX root=../paper.tex
\begin{figure*}[t]
\centering
% \includegraphics[width=\linewidth]{assets/ddg-depth.pdf}
\includegraphics[width=\linewidth]{assets/entropy-rate-cpp.pdf}
\captionsetup{size=footnotesize, skip=0pt}
\caption{Comparison of sampling rate (samples per wall-clock second)
  and order of growth of FLDR
  (Algorithm~\ref{alg:rejection-dyadic-ddg}) with linear inversion sampling
  (GNU C++ library~\citep{devroye1986,lea1992})
  and alias sampling (Boost C++ library~\citep{walker1977general,schling2011}).}
\label{fig:entropy-rate-cpp}
\medskip

\captionsetup{size=footnotesize, skip=0pt}
\captionof{table}{Comparison of wall-clock time and number of calls to
  underling pseudo-random number generator to generate one million
  samples from $1000$ dimensional distributions (panel 3 of
  Fig.~\ref{fig:entropy-rate-cpp}) using FLDR and baseline
  samplers.}
\label{tab:entropy-rate-cpp}
\footnotesize
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrr}
\toprule
Method
  & Target Dist. Entropy (Bits)
  & No. of PRNG Calls
  & PRNG Wall-Clock Time (ms)
  \\ \midrule
\multirow{5}{*}{
  \shortstack[l]{Fast Loaded Dice Roller \\
    (FLDR; Algorithm ~\ref{alg:rejection-dyadic-ddg})}}
  % & 1 & 123,607 & 3.69 \\
~ & 2 & 165,335 & 3.88 \\
% ~ & 3 & 182,839 & 4.27 \\
~ & 4 & 234,443 & 6.08 \\
% ~ & 5 & 258,786 & 5.66 \\
~ & 6 & 288,997 & 8.60 \\
% ~ & 7 & 325,781 & 8.54 \\
~ & 8 & 352,015 & 9.10 \\
% ~ & 9 & 383,138 & 8.42 \\
~ & 10 & 412,676 & 7.78 \\ \midrule
Baseline C++ Samplers \\
(Boost/Alias; GNU/Inversion) & (all) & 1,000,000 & 21.50 \\ \bottomrule
\end{tabular*}
\end{figure*}

